GO-DICE: Goal-Conditioned Option-Aware Offline Imitation Learning via Stationary Distribution Correction Estimation

Offline imitation learning (IL) refers to learning expert behavior solely from demonstrations, without any additional interaction with the environment. Despite significant advances in offline IL, existing techniques find it challenging to learn policies for long-horizon tasks and require significant re-training when task specifications change. Towards addressing these limitations, we present GO-DICE an offline IL technique for goal-conditioned long-horizon sequential tasks. GO-DICE discerns a hierarchy of sub-tasks from demonstrations and uses these to learn separate policies for sub-task transitions and action execution, respectively; this hierarchical policy learning facilitates long-horizon reasoning. Inspired by the expansive DICE-family of techniques, policy learning at both the levels transpires within the space of stationary distributions. Further, both policies are learnt with goal conditioning to minimize need for retraining when task goals change. Experimental results substantiate that GO-DICE outperforms recent baselines, as evidenced by a marked improvement in the completion rate of increasingly challenging pick-and-place Mujoco robotic tasks. GO-DICE is also capable of leveraging imperfect demonstration and partial task segmentation when available, both of which boost task performance relative to learning from expert demonstrations alone.

==> text/method.tex <==
\section{\approach -- Version 1}

\begin{algorithm}
\caption{\approach for offline imitation learning}
\label{alg:godice}
\begin{algorithmic}[1]
\Require Expert trajectories $\mathcal{D}_E$, imperfect trajectories $\mathcal{D}_I$
\Ensure Learned policy $\Tilde{\pi} = \{\pi_H, \pi_L\}$
\State \textbf{Parameters:} \textsc{Unsupervised}, $N, N_{sync}, \lambda$
\For{$n = 1$ to $N$}
    \If{$n \mod N_{sync} == 0$}
        \State $\Tilde{\pi}'\gets \lambda\Tilde{\pi}' + (1-\lambda)\Tilde{\pi}$ \Comment{Update target networks}
        \State Segment imperfect trajectories using Eq.\ref{eq:Viterbi}
        \If{\textsc{Unsupervised}}
            \State Segment expert trajectories using Eq.\ref{eq:Viterbi}
        \EndIf
    \EndIf
    \State Update discriminator $\Psi$ using Eq.\ref{eq:disc_func_objective}
    \State Update value function $\nu$ using Eq.\ref{eq:value_func_objective}
    \State Update policy $\Tilde{\pi}$ using Eq.\ref{eq:policy_func_objective}
\EndFor
\end{algorithmic}
\end{algorithm}


We introduce \approach, termed as \textit{Goal-Conditioned Option-aware Stationary Distribution Correction Estimation}. This method augments the recent DICE family of offline imitation learning techniques by integrating them into an options framework. To achieve this, we transform the original convex optimization problem into its Dual formulation. This transformation enables us to derive closed-form solutions for policy estimation without the need for on-policy sampling.

\vu{Add 1-2 sentences about why we are building upon DICE: 
Given the task segmentations and choice of policy representation, in theory, any offline IL technique could be used as a starting point to instantiate the policy learning subroutines.}
\vu{RESOLVED:The methodology also needs to describe the reason behind why you are doing this analysis. Why these particular steps?}
\vu{RESOLVED: Insert 1-2 sentences on Why do we need to convert primal to dual?}

\subsection{Primal to Dual Conversion}

For tractable optimization in the offline setting, we first convert the constrained optimisation problem (\ref{eq:il_dist_match_reg}) into unconstrained using the method of Lagrangian multipliers. We obtain the following saddle point optimisation over the Lagrangian function $\mathcal{L}$.

\begin{align}
     \max_{d^{\Tilde{\pi}}\geq0}\min_{\nu}\;  &\mathcal{L}(d^{\Tilde{\pi}}, \nu) = \nonumber\\ 
     & - D_{KL}(d^{\Tilde{\pi}}||d^{\pi_E}) - \alpha D_{KL}(d^{\Tilde{\pi}}||d^{\pi_O}) \nonumber\\
     &+ \sum_{c',s,g}\nu(c',s,g)\bigg((1-\gamma)\Tilde{\mu}(c', s; g) \nonumber\\
     &+ \gamma (T_*d^{\widetilde{\pi}})(c',s, g) - \sum_{c, a} d^{\widetilde{\pi}}(c', s, c, a; g)\bigg)
\label{eq:lagrangian function}
\end{align}

where, $\nu(c', s, g)$ are the Lagrangian multipliers for all $(c', s, g)$. $T_*$ is the transposed Bellman operator such that $(T_*d)(c',s; g) = \sum_{c'', s', a'}\mathbf{T}(s|s',a')d(c'', s', c', a'; g)$. Now we rearrange the terms in the objective (\ref{eq:lagrangian function}) to re-formulate the Lagrangian in terms of the stationary distribution ratio $w(c',s,c,a, g) = \frac{d^{\Tilde{\pi}}(c',s,c,a; g)}{d^{\pi_O}(c',s,c,a; g)}$.

\begin{align}
   \max_{w\geq 0}\min_{\nu} \; & \mathcal{L}(w, \nu;r) = \nonumber\\
   &(1-\gamma)\mathbb{E}_{(c',s)\sim \Tilde{\mu}}[\nu(c',s,g)] \nonumber\\
   &+ \mathbb{E}_{(c',s,c,a)\sim d^{\pi_O}}\Big[w(c',s,c,a, g)\big(A_{\nu}(c',s,c,a, g) \nonumber\\  
   &- (1+\alpha)\log w(c',s,c,a, g)\big)\Big]
   \label{eq:new lagrangian function}
\end{align}

where, for the given reward function $r$ estimating the log-distribution ratio of expert and offline $\log\frac{d^{\pi_E}(c',s,c,a; g)}{d^{\pi_O}(c',s,c,a; g)}$, $A_{\nu}=r(c',s,c,a, g)+\gamma (T\nu)(s, c, a, g) - \nu(c',s, g) $ resembles the commonly observed Advantage function of reinforcement learning \cite{?}. Thus in Dice-family, the Lagrangian multiplier $\nu$ is also referred to as the `Critic'. $(T\nu)(c',s, c, a;g)=\sum_{s'} \mathbf{T}(s'|s, a)\nu(c, s', g)$ is the adjoint of transposed Bellman operator $T_{*}$ such that $\sum_{s'}\nu(c, s', g)(T_*d)(c, s', g) = \sum_{c's,a}d(c',s,c,a;g)(T\nu)(s, c, a, g)$. The derivation of (\ref{eq:new lagrangian function}) can be found in the Appendix \ref{??}.
 
Now, assuming a stationary distribution satisfies the Bellman constraints \ref{eq:bellman_constraint}, we infer the existence of a strict feasible point for the convex optimization problem described in \ref{eq:il_dist_match_reg}. With this assumption, Slater's conditions are met, ensuring strong duality. Consequently, the order of min-max can be interchanged, and the primal's optimal value in (\ref{eq:new) lagrangian function} is attained using its dual formulation.

\begin{align}
   \min_{\nu} \max_{w\geq 0} \; & \mathcal{L}(w, \nu;r)
   \label{eq:dual}
\end{align}

The closed-form solution of inner maximum optimization provides optimal importance weights: 
\begin{align}
    \frac{d^{\Tilde{\pi}*}(c',s,c,a; g)}{d^{\pi_O}(c',s,c,a, g)} = w^*(c',s,c,a; g) = \exp(\frac{A_{\nu}}{1+\alpha}-1)
   \label{eq:optimal_imp_weight}
\end{align}

\textbf{Dual Value Function Objective.} Using optimal importance weights, the overall optimization (\ref{eq:dual}) reduces to convex minimization over the value function $\nu(c',s, g)$:
\begin{align}
    \min_{\nu(c',s,g)}\; & \mathcal{L}(w^*, \nu;r) = \nonumber\\
    & (1-\gamma)\mathbb{E}_{(c',s)\sim p_o}[\nu(c',s;g)] \nonumber\\
    & + (1+\alpha)\mathbb{E}_{(c',s,c,a)\sim d^{\pi_O}}[\exp(\frac{A_{\nu}}{1+\alpha}-1)]
    \label{eq:value_func_objective_unstable}
\end{align}

We can observe that optimising the formulation is unstable due to presence of exponential term which is prone to gradient explosion. Hence, similar to \cite{kim2021demodice} we use the following surrogate objective instead to impart stability during training:

\begin{align}
    \min_{\nu(c',s;g)} & \; \hat{\mathcal{L}}(w^*, \nu;r) = \nonumber\\
     & (1-\gamma)\mathbb{E}_{(c',s)\sim p_o}[\nu(c',s;g)] \nonumber \\
    &+ (1+\alpha)\log\mathbb{E}_{(c',s,c,a)\sim d^{\pi_O}}[\exp(\frac{A_{\nu}}{1+\alpha})]
    \label{eq:value_func_objective}
\end{align}
The objective is still convex w.r.t $\nu$ and shares the same optimal value with $\mathcal{L}$. The proof can be found in the Appendix.


\textbf{Discriminator Objective.} To estimate the log-distribution ratio $r = \log\frac{d^{\pi_E}(c',s,c,a; g)}{d^{\pi_O}(c',s,c,a; g)}$, we train a Discriminator network $\Psi : \mathcal{C}\times\mathcal{S}\times\mathcal{C}\times\mathcal{A}\times\mathcal{G}\mapsto (0,1)$ with the following objective:
\begin{align}
    \min \quad &\mathbb{E}_{d^{\pi_E}}[\log\Psi(c', s, c, a;g)]\nonumber\\
    + &\mathbb{E}_{d^{\pi_O}}[\log(1-\Psi(c', s, c, a ; g)]
    \label{eq:disc_func_objective}
\end{align}
It can be observed that the optimal value achieved by optimising the objective is $\Psi^*=\frac{d^{\pi_O}}{d^{\pi_O} + d^{\pi_E}}$ can be used to estimate the required log-distribution ratio $r = -\log\Big(\frac{1}{\Psi^*} - 1\Big)$.



\textbf{Weighted Policy Regression.} Finally using the optimal importance weights  $w^*(c',s,c,a; g) = \frac{d^{\Tilde{\pi}^*}(c',s,c,a; g)}{d^{\pi_O}(c',s,c,a; g)}$ we can do weighted-behavior cloning to learn the high- and low-level policy weights:
\begin{align}
    \max\mathbb{E}_{g\sim p(g), (c',s,c,a)\sim d^{\Tilde{\pi}^*}}&\big[\log\Tilde{\pi}(c, a|s,c',g)\big]\nonumber\\
    \max\mathbb{E}_{g\sim p(g), (c',s,c,a)\sim d^{\Tilde{\pi}^*}}&\big[\log\pi_H(c|s,c',g\nonumber)\\
    &+\log\pi_L(a|s,c,g)\big]\nonumber\\
    \max\mathbb{E}_{g\sim p(g), (c',s,c,a)\sim d^{{\pi}_O}}&\bigg[w^*(c',s,c,a;g)\Big(\log\pi_H(c|s,c',g)\nonumber\\
    &+\log\pi_L(a|s,c,g)\Big)\bigg]
    \label{eq:policy_func_objective}
\end{align}


\subsection{Option Inference for Trajectory Segmentation} 
So far we have assumed the availability of option annotations for each trajectory in the dataset. Such an assumption is impractical. By observing that the overall transition system follows a Hidden Markov Model \cite{?}, we use Viterbi decoding to infer the sequence of options $c_{0:T-1}$ and segment the trajectories given observed sequence of state and actions $(s_{0:T}, a_{0:T-1})$ where $\pi_H$ represents the transition probability and $\pi_L$ represents the emission probability.

\begin{align*}
    \hat{c}_{0:T-1} = arg\max p(s_{0:T}, a_{0:T-1}, c_{0:T-1}; g)
\end{align*}

To find the most-likely options, following recursive formulation is used.
\begin{align}
    \hat{\mu}(c_t) & = \max_{c_{t-1}}\hat{\mu}_(c_{t-1})+ \log\pi_H'(c_t|s_t, c_{t-1}, g) \nonumber\\
    &+ \log\pi_L'(a_t|s_t, c_t, g)
\label{eq:Viterbi}
\end{align}

where, $(\pi_H', \pi_L')$ denote the target high- and low-level policy networks, which are periodically synchronized with the main networks $(\pi_H, \pi_L)$ using Polyak averaging. These primary networks are trained employing the \approach methodology, as detailed in Algorithm \ref{alg:godice}. Most often, provided trajectories lack supervision over options. Thus, they are decoded using the policy networks. However, these inferred options serve as input to train the policy networks which could destabilise the learning. Thus use of target networks enhances stability and foster convergence in the learning process, a mechanism most commonly used by algorithms like DDQN.

Distinctively, in the context of \approach, the periodic variations in the options inferred for trajectories mean that the objectives for the Discriminator, Value Function, and Policy are intertwined since now the annotated $(c',c)$ values for a given state-action pair are dynamic. This characteristic differentiates \approach from other members of the DICE-family \citep{kim2021demodice, ma2022versatile, ma2022offline}, underscoring its unique approach to the problem.


